DIAR: Removing Uninteresting Bytes from Seeds in Software Fuzzing

Software fuzzing mutates bytes in the test seeds to explore different behaviors of the program under test. Initial seeds can have great impact on the performance of a fuzzing campaign. Mutating a lot of uninteresting bytes in a large seed wastes the fuzzing resources. In this paper, we present the preliminary results of our approach that aims to improve the performance of fuzzers through identifying and removing uninteresting bytes in the seeds. In particular, we present DIAR, a technique that reduces the size of the seeds based on their coverage. Our preliminary results suggest fuzzing campaigns that start with reduced seeds, find new paths faster, and can produce higher coverage overall.

==> tool-arch.tex <==
\section{Tool Architecture}
\label{tool-arch}
In this section, we provide an overview of the architecture of \tool.
We also present information on its usage and performance.
 The implementation and documentation of \tool is available in Github\footnote{\url{https://github.com/AftabHussain/afl-test-viz}}.

Figure~\ref{fig-workflow} depicts the architecture of \tool and its main components, which are: Test Input Color Representation Generator and Test Input Image Generator. 

\begin{figure}
\centering
\begin{minipage}[t]{.6\textwidth}
  \centering
   \def\svgscale{0.38}
  \includesvg{figs/afl-vis-overview.svg}
  \captionof{figure}{Overview of \tool.}
  \label{fig-workflow}
\end{minipage}%
\begin{minipage}[t]{.3\textwidth}
  \centering
   \def\svgscale{0.54}
  \includesvg{figs/afl-sample-op.svg}
  \captionof{figure}{Cropped sample image of a test input.}
  \label{fig-sample-op}
\end{minipage}
\end{figure}
Figure~\ref{fig-sample-op} shows a sample visualization output of \tool of a test input. 

% For each test input $t_{i+1}$ derived by mutation of test input $t_i$, an image of $t$ is generated such that each byte of $t$ is encoded as a color in hexadecimal format. 

\subsection{Extracting Color Representations of Test Inputs} 
\tool extends AFL to capture the byte stream representations of new test inputs that are generated as AFL mutates original seeds (Figure~\ref{fig-parts}(a)). 
%The test input byte code generation phase 
% (Fig.~\ref{fig-parts}(a)) captures the byte stream representation of tests generated by AFL through mutation.
\tool saves these representations in a single file (a dump file in hexadecimal). Each byte's hex code is chosen to represent a shade of red, depending on the value stored in the byte (we elaborate on the color representation in the following subsection). 
Each line of this file corresponds to the representation of a single test input. 
%This component has of our tool is implemented as a patch in AFL.

\subsection{Test Input Image Generator} 
This piece of our tool (Fig.~\ref{fig-parts}(b)), written in Python, reads the file generated by the color representation generator, line by line, and generates PNG image files (where each line corresponds to a test input as mentioned previously). 
In the image output, each box represents a byte of a test input. 
For obtaining the box colors we use the six-digit hex triplet, a three-byte hexadecimal number, which is typically used for various computing applications, e.g. html, svg, etc., to generate colors. Each of these three bytes show the red, green, and blue components of the color respectively~\cite{hex-trip}. The box color representation for each byte of the test input is evaluated as follows: byte $xy$ is translated to the hex color code $xy0000$, where $xy$ is a hex representation of a test input byte, where $x$ and $y$ each belong to the set of 16 hexadecimal symbols ($0-9$, $A-F$). The box dimensions can be changed to vary the number of test input bytes to display in the image.
The PNG files can be used independently to represent individual test inputs, or can be used to generate a time-lapse video of the evolution of the test inputs using a linear image interpolator~\cite{lin-img-interpolator}, or a screen recorder~\cite{simplescreenrec}.

% \texttt{ffmpeg}~\cite{?}\Fix{add citation}.

\begin{figure}[htbp]
  \centering
  %\def\svgscale{0.55}
  \def\svgwidth{\columnwidth}
  \includesvg{figs/afl-viz-parts.svg}
  \caption{Workflow of the \tool Tool. (a) Test Input Color Representation Generation. (b) Test Input Image Generation}
  \label{fig-parts}
\end{figure}

%if a byte is, say, 7c, then the hex color code is #7c0000. The implementation is in viz_tests.py, provided in the code folder.

\subsection{Usage and Performance Considerations}

The present implementation is adapted for an AFL fuzzing campaign with a single test input. Although the overhead of writing to the color dump file is minimal during the fuzzing campaign, since a single file is used, the file can get very large over long fuzzing periods.
We are considering to extend \tool to optimize the storage use through using a more compressed representation of the test inputs.

